Higher-dimensional O'Grady's resolutions and their exceptional locus

For any $n \ge 3$, we consider the moduli space $M_n$ of semistable sheaves with Mukai vector $2(1,0,1-n)$ on a K3 surface. The moduli space $M_n$ is singular and lacks a crepant resolution, but might still admit a categorical crepant one. As a preliminary to exploring this possibility, we study the explicit resolution of singularities of $M_n$ constructed by O'Grady, and provide a global description of its exceptional locus.

==> main.bib.tex <==
@article {AcHKc,
    AUTHOR = {Abuaf, R.},
     TITLE = {Compact hyper-{K}ähler categories},
     NOTE = {With an appendix by Gr\'egoire Menet},
   JOURNAL = {Ann. Sc. Norm. Super. Pisa Cl. Sci. (5)},
  FJOURNAL = {Annali della Scuola Normale Superiore di Scienze. Serie V},
    VOLUME = {23},
      YEAR = {2022},
    NUMBER = {3},
     PAGES = {1525--1563},
      ISSN = {0391-173X,2036-2145},
   MRCLASS = {14F08 (14E15 14J30 14J42)},
  MRNUMBER = {4497753},
MRREVIEWER = {Adrian\ Langer},
}

@article {ASsmssK3snqv,
    AUTHOR = {Arbarello, E. and Saccà, G.},
     TITLE = {Singularities of moduli spaces of sheaves on {K}3 surfaces and {N}akajima quiver varieties},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in mathematics},
    VOLUME = {329},
      YEAR = {2018},
    NUMBER = {},
     PAGES = {649--703},
      ISSN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {Alan\ Matthew\ Thompson},
       DOI = {10.1016/j.aim.2018.02.003},
       URL = {https://doi.org/10.1016/j.aim.2018.02.003},
}

@article {BMMfcmsKd0,
    AUTHOR = {Bandiera, R. and Manetti, M. and Meazzini, F.},
     TITLE = {Formality conjecture for minimal surfaces of {K}odaira dimension 0},
   JOURNAL = {Compos. Math.},
  FJOURNAL = {Compositio Mathematica},
    VOLUME = {157},
      YEAR = {2021},
    NUMBER = {2},
     PAGES = {215--235},
      ISSN = {0010-437X,1570-5846},
   MRCLASS = {14F08 (14D15 14J28 16E45 18G10 18G15)},
  MRNUMBER = {4219218},
MRREVIEWER = {Chunyi\ Li},
       DOI = {10.1112/s0010437x20007605},
       URL = {https://doi.org/10.1112/s0010437x20007605},
}

@article {Bss,
    AUTHOR = {Beauville, A.},
     TITLE = {Symplectic singularities},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {139},
      YEAR = {2000},
    NUMBER = {3},
     PAGES = {541--549},
      ISSN = {0020-9910,1432-1297},
   MRCLASS = {14B05 (14E15 32S45)},
  MRNUMBER = {1738060},
MRREVIEWER = {Marko\ Roczen},
       DOI = {10.1007/s002229900043},
       URL = {https://doi.org/10.1007/s002229900043},
}

@Book{BSUlsagga,
 Author = {Brion, M. and Samuel, P. and Uma, V.},
 Title = {Lectures on the structure of algebraic groups and geometric applications},
 Edition = {},
 FSeries = {CMI Lecture Series in Mathematics},
 Series = {CMI Lecture Ser. Math.},
 Volume = {1},
 ISBN = {978-93-86279-58-3},
 Year = {2013},
 Publisher = {Hindustan Book Agency Gurgaon},
 Language = {English},
 Keywords = {},
 zbMATH = {},
 Zbl = {}
}

@article {BZfcK3s,
    AUTHOR = {Budur, N. and Zhang, Z.},
     TITLE = {Formality conjecture for {K}3 surfaces},
   JOURNAL = {Compos. Math.},
  FJOURNAL = {Compositio Mathematica},
    VOLUME = {155},
      YEAR = {2019},
    NUMBER = {5},
     PAGES = {902--911},
      ISSN = {0010-437X,1570-5846},
   MRCLASS = {14F05 (14J28 16E45)},
  MRNUMBER = {3942159},
MRREVIEWER = {Richard\ P.\ Thomas},
       DOI = {10.1112/s0010437x19007206},
       URL = {https://doi.org/10.1112/s0010437x19007206},
}

@article {ChoyKiem,
    AUTHOR = {Choy, J. and Kiem, Y.-H.},
     TITLE = {Nonexistence of a crepant resolution of some moduli spaces of sheaves on a {K}3 surface},
   JOURNAL = {J. Korean Math. Soc.},
  FJOURNAL = {Journal of the Korean Mathematical Society},
    VOLUME = {44},
      YEAR = {2007},
    NUMBER = {1},
     PAGES = {35--54},
      ISSN = {0304-9914,2234-3008},
   MRCLASS = {14D20 (14J28 14J60)},
  MRNUMBER = {2283459},
MRREVIEWER = {Nicolas\ Perrin},
       DOI = {10.4134/JKMS.2007.44.1.035},
       URL = {https://doi.org/10.4134/JKMS.2007.44.1.035},
}

@book {Fit,
    AUTHOR = {Fulton, W.},
     TITLE = {Intersection theory},
    SERIES = {Ergebnisse der Mathematik und ihrer Grenzgebiete. 3. Folge. A
              Series of Modern Surveys in Mathematics},
    VOLUME = {2},
   EDITION = {Second},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1998},
     PAGES = {xiv+470},
      ISBN = {3-540-62046-X; 0-387-98549-2},
   MRCLASS = {14C17 (14-02)},
  MRNUMBER = {1644323},
       DOI = {10.1007/978-1-4612-1700-8},
       URL = {https://doi.org/10.1007/978-1-4612-1700-8},
}

@Book{EGA,
 Author = {Grothendieck, A.},
 Title = {Éléments de géométrie algébrique (rédigés avec la collaboration de J.\ Dieudonné)},
 Edition = {},
 FSeries = {},
 Series = {},
 Volume = {},
 ISBN = {},
 Year = {1960-1967},
 Publisher = {Publ. Math. IHÉS},
 Language = {},
 Keywords = {},
 zbMATH = {},
 Zbl = {}
}

@book {Rag,
    AUTHOR = {Hartshorne, R.},
     TITLE = {Algebraic {G}eometry},
    SERIES = {Graduate Texts in Mathematics, No. 52},
 PUBLISHER = {Springer-Verlag, New York-Heidelberg},
      YEAR = {1977},
     PAGES = {xvi+496},
      ISBN = {0-387-90244-9},
   MRCLASS = {14-01},
  MRNUMBER = {0463157},
MRREVIEWER = {Robert Speiser},
}

@book {HOIebu,
    AUTHOR = {Herrmann, M. and Ikeda, S. and Orbanz, U.},
     TITLE = {Equimultiplicity and {B}lowing up. An {A}lgebraic {S}tudy},
	NOTE = {With an Appendix by B.\ Moonen},
    SERIES = {},
 PUBLISHER = {Springer-Verlag, Berlin-Heidelberg},
      YEAR = {1988},
     PAGES = {xviii+629},
      ISBN = {3-540-15289-X},
   MRCLASS = {13H15, 13H10, 14B15, 32B30},
  MRNUMBER = {0954831},
MRREVIEWER = {Bădescu, L.},
}

@book{huybrechts2006fourier,
  title={Fourier--{M}ukai transforms in algebraic geometry},
  author={Huybrechts, D.},
  year={2006},
  publisher={Clarendon Press, Oxford}
}

@book{HLgmss,
  title={The geometry of moduli spaces of sheaves, 2nd edition},
  author={Huybrechts, D. and Lehn, M.},
  year={2010},
  publisher={Cambridge University Press}
}

@article {Ispct,
    AUTHOR = {Ishii, S.},
     TITLE = {Some projective contraction theorems},
   JOURNAL = {Manuscripta math.},
  FJOURNAL = {Manuscripta mathematica},
    VOLUME = {22},
      YEAR = {1977},
    NUMBER = {},
     PAGES = {343--358},
      ISSN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
       DOI = {10.1007/BF01168221},
       URL = {https://doi.org/10.1007/BF01168221},
}

@article {KLSssms,
    AUTHOR = {Kaledin, D. and Lehn, M. and Sorger, Ch.},
     TITLE = {Singular symplectic moduli spaces},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones mathematicae},
    VOLUME = {164},
      YEAR = {2006},
    NUMBER = {3},
     PAGES = {591--614},
      ISSN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
       DOI = {10.1007/s00222-005-0484-6},
       URL = { https://doi-org.ezproxy.universite-paris-saclay.fr/10.1007/s00222-005-0484-6},
}

@article {KPdqnvBn,
    AUTHOR = {Kirwan, F. C.},
     TITLE = {Partial desingularisations of quotients of nonsingular varieties and their {B}etti numbers},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {122},
      YEAR = {1985},
    NUMBER = {1},
     PAGES = {41--85},
      ISSN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
       DOI = {10.2307/1971369},
       URL = {https://doi.org/10.2307/1971369}}

@Book{KSSATI,
 Author = {Kraft, H. and Slodowy, P. and Springer, T. A.},
 Title = {Algebraische {T}ransformationsgruppen und {I}nvariantentheorie},
 Edition = {},
 FSeries = {},
 Series = {DMV Seminar},
 Volume = {13},
 ISBN = {3-7643-2284-5},
 Year = {1989},
 Publisher = {Birkh\"auser Verlag, Basel},
 Language = {German},
 Keywords = {},
 zbMATH = {},
 Zbl = {}
}

@article {Ket,
    AUTHOR = {Kuznetsov, A. G.},
     TITLE = {Hyperplane sections and derived categories},
   JOURNAL = {Izv. Ross. Akad. Nauk Ser. Mat.},
  FJOURNAL = {Izvestiya Rossiiskoi Akademii Nauk. Seriya Matematicheskaya},
    VOLUME = {70},
      YEAR = {2006},
    NUMBER = {3},
     PAGES = {23--128},
      ISSN = {1607-0046},
   MRCLASS = {14F05 (18E30)},
  MRNUMBER = {2238172},
MRREVIEWER = {Andrei D. Halanay},
       DOI = {10.1070/IM2006v070n03ABEH002318},
       URL = {https://0-doi-org.pugwash.lib.warwick.ac.uk/10.1070/IM2006v070n03ABEH002318},
}

@article {Kldcr,
    AUTHOR = {Kuznetsov, A. G.},
     TITLE = {Lefschetz decompositions and categorical resolutions of
              singularities},
   JOURNAL = {Selecta Math. (N.S.)},
  FJOURNAL = {Selecta Mathematica. New Series},
    VOLUME = {13},
      YEAR = {2008},
    NUMBER = {4},
     PAGES = {661--696},
      ISSN = {1022-1824},
   MRCLASS = {18E30 (14E15)},
  MRNUMBER = {2403307},
MRREVIEWER = {Emanuele Macr\'{\i}},
       DOI = {10.1007/s00029-008-0052-1},
       URL = {https://0-doi-org.pugwash.lib.warwick.ac.uk/10.1007/s00029-008-0052-1},
}

@article {LBtrg2x2m,
    AUTHOR = {Le Bruyn, L.},
     TITLE = {Trace rings of generic {$2$} by {$2$} matrices},
   JOURNAL = {Mem. Amer. Math. Soc.},
  FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {66},
      YEAR = {1987},
    NUMBER = {363},
     PAGES = {vi--100},
      ISSN = {0065-9266, 1947-6221},
   MRCLASS = {16A38 (11E88 15A66 16A42)},
  MRNUMBER = {878906},
MRREVIEWER = {E.\ Formanek},
       DOI = {10.1090/memo/0363},
       URL = {https://doi.org/10.1090/memo/0363},
}

@article {LcsQs,
    AUTHOR = {Lehn, M.},
     TITLE = {On the cotangent sheaf of {Q}uot-schemes},
   JOURNAL = {Int.\ J.\ Math.},
  FJOURNAL = {International journal of mathematics},
    VOLUME = {9},
      YEAR = {1998},
    NUMBER = {4},
     PAGES = {513--522},
      ISSN = {},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
       DOI = {10.1142/S0129167X98000221},
       URL = { https://doi-org.ezproxy.universite-paris-saclay.fr/10.1142/S0129167X98000221},
}

@article {LSsO'G,
    AUTHOR = {Lehn, M. and Sorger, Ch.},
     TITLE = {La singularité de {O}’{G}rady},
   JOURNAL = {J. Algebraic Geom.},
  FJOURNAL = {Journal of Algebraic Geometry},
    VOLUME = {15},
      YEAR = {2006},
    NUMBER = {4},
     PAGES = {753--770},
      ISSN = {1534-7486},
   MRCLASS = {14D20 (14E15)},
  MRNUMBER = {2237269},
MRREVIEWER = {Jean-Marc Drézet},
       DOI = {10.1090/S1056-3911-06-00437-1},
       URL = { https://doi-org.ezproxy.universite-paris-saclay.fr/10.1090/S1056-3911-06-00437-1},
}
@article {MBBccc,
    AUTHOR = {Markman, E.},
     TITLE = {The {B}eauville-{B}ogomolov class as a characteristic class},
   JOURNAL = {J.\ Algebraic Geom.},
  FJOURNAL = {Journal of algebraic geometry},
    VOLUME = {29},
      YEAR = {2020},
    NUMBER = {2},
     PAGES = {199--245},
      ISSN = {1534-7486},
   MRCLASS = {},
  MRNUMBER = {MR4069649},
MRREVIEWER = {Kieran G. O'Grady},
       DOI = {10.1090/jag/750},
       URL = {https://doi-org.ezproxy.universite-paris-saclay.fr/10.1090/jag/750}}

@misc{MABBccc,
    shorthand    = {},
    author       = {Markman, E.},
    title        = {Appendix to ``The {B}eauville-{B}ogomolov class as a characteristic class''},
    howpublished = {\url{https://people.math.umass.edu/~markman/appendix100508.pdf}},
    year         = {2010},
}

@article {Mgcrmssss,
    AUTHOR = {Markman, E.},
     TITLE = {Generators of the cohomology ring of moduli spaces of sheaves on symplectic surfaces},
   JOURNAL = {J.\ reine angew. Math.},
  FJOURNAL = {Journal für die reine und angewandte Mathematik},
    VOLUME = {544},
      YEAR = {2002},
    NUMBER = {},
     PAGES = {61--82},
      ISSN = {},
   MRCLASS = {14D20,14J28,14J60},
  MRNUMBER = {MR1887889},
MRREVIEWER = {},
       DOI = {10.1515/crll.2002.028},
       URL = {https://doi-org.ezproxy.universite-paris-saclay.fr/10.1515/crll.2002.028}}

@article {O'GdmsK3,
    AUTHOR = {O'Grady, K. G.},
     TITLE = {Desingularized moduli spaces of sheaves on a {K}3},
   JOURNAL = {J.\ reine angew. Math.},
  FJOURNAL = {Journal für die reine und angewandte Mathematik},
    VOLUME = {512},
      YEAR = {1999},
    NUMBER = {},
     PAGES = {47--117},
      ISSN = {0075-4102},
   MRCLASS = {},
  MRNUMBER = {},
MRREVIEWER = {},
       DOI = {10.1515/crll.1999.056},
       URL = {https://www-degruyter-com.ezproxy.universite-paris-saclay.fr/document/document/doi/10.1515/crll.1999.056}}

@article{O'GdmsK3I,
  AUTHOR = {O'Grady, K. G.},
     TITLE = {Desingularized moduli spaces of sheaves on a {K}3 {I}},
  journal={arXiv:alg-geom/9708009v2},
  volume={},
  number={},
  pages={},
  year={1998},
  publisher={}
}

@incollection {SSaT,
    AUTHOR = {Slodowy, P.},
     TITLE = {Der {S}cheibensatz f\"ur algebraische {T}ransformationsgruppen},
   BOOKTITLE = {Algebraische {T}ransformationsgruppen und {I}nvariantentheorie},
  SERIES = {DMV Sem.},
    VOLUME = {13},
PAGES = {89--113},
 PUBLISHER = {Birkh\"auser, Basel},
      YEAR = {1989},     
      ISBN = {3-7643-2284-5},
   MRCLASS = {14L30},
  MRNUMBER = {1044587},
}
